Integrating LLMs in Software Engineering Education: Motivators, Demotivators, and a Roadmap Towards a Framework for Finnish Higher Education Institutes

The increasing adoption of Large Language Models (LLMs) in software engineering education presents both opportunities and challenges. While LLMs offer benefits such as enhanced learning experiences, automated assessments, and personalized tutoring, their integration also raises concerns about academic integrity, student over-reliance, and ethical considerations. In this study, we conducted a preliminary literature review to identify motivators and demotivators for using LLMs in software engineering education. We applied a thematic mapping process to categorize and structure these factors (motivators and demotivators), offering a comprehensive view of their impact. In total, we identified 25 motivators and 30 demotivators, which are further organized into four high-level themes. This mapping provides a structured framework for understanding the factors that influence the integration of LLMs in software engineering education, both positively and negatively. As part of a larger research project, this study serves as a feasibility assessment, laying the groundwork for future systematic literature review and empirical studies. Ultimately, this project aims to develop a framework to assist Finnish higher education institutions in effectively integrating LLMs into software engineering education while addressing potential risks and challenges.

==> Threats_to_Validity.tex <==
\section{Threats to Validity} \label{Sec:Threat_Validity)}
Various threats could affect the validity of the study findings. In this study, we analyzed the potential threats in four main categories—internal, external, construct, and conclusion validity—as defined by Wohlin \cite{wohlin2012experimentation}.

\subsection{Internal Validity}
Internal validity refers to whether the observed results are truly caused by the investigated factors rather than external influences. In this study, potential biases in data selection, researcher interpretations, and thematic mapping could pose threats. Additionally, using a traditional literature review instead of a systematic review (SLR) increases the risk of selection bias, incomplete coverage, and limited reproducibility. To mitigate these threats, we applied systematic data coding, cross-validated findings with external reviewers, documented the review process step by step, and assessed interpersonal bias using Kendall’s coefficient of concordance analysis.

\subsection{External Validity}
External validity refers to the extent to which the study findings can be generalized. In this study, the identified motivators and demotivators were derived from a traditional literature review, which may limit the breadth of included studies. Additionally, the thematic mapping, while structured, is influenced by selected studies and may not capture all possible themes. To mitigate this, we ensured diverse sources, followed a structured review process, and validated the thematic mapping through a formal thematic approach and multiple reviewers (authors) to reduce bias.

\subsection{Construct Validity} 
Construct validity assesses whether the study accurately measures the intended concepts. In this study, threats may arise from misclassification of motivators and demotivators or inconsistencies in thematic mapping, which could affect the reliability of identified themes. To mitigate this, we followed a formal thematic analysis process, used clearly defined coding schemes, and involved multiple reviewers to ensure consistency and reduce subjective bias.

\subsection{Conclusion Validity}
Conclusion validity ensures that the study’s findings and inferences are logically sound and well-supported by the data. Threats in this study may arise from biases in data interpretation, limited dataset coverage, or overfitting of thematic patterns, potentially leading to misleading conclusions. To mitigate these threats, we followed a structured review process, critically evaluated emerging patterns through consensus meetings among all authors, and ensured clear documentation of the review process, including a replication package \cite{khan2025motivators} for transparency and reproducibility.
